Almost-Matching-Exactly for Treatment Effect Estimation under Network Interference

We propose a matching method that recovers direct treatment effects from randomized experiments where units are connected in an observed network, and units that share edges can potentially influence each others' outcomes. Traditional treatment effect estimators for randomized experiments are biased and error prone in this setting. Our method matches units almost exactly on counts of unique subgraphs within their neighborhood graphs. The matches that we construct are interpretable and high-quality. Our method can be extended easily to accommodate additional unit-level covariate information. We show empirically that our method performs better than other existing methodologies for this problem, while producing meaningful, interpretable results.

==> additive_interference_old.tex <==
Here, we use an additive interference function in our outcomes: $Y_i(t, \btnoti) = t\tau_i + \sum_{p = 1}^P \gamma_pm_p + \epsilon_i$, where each component is weighted differently. The weights for each of our experimental settings are given in Table \ref{Tab:SettingsAdditive}. For this experiment we have 50 units connected in a $ER(50, 0.1)$ graph, with 25 treated.
\begin{table}[!htbp]
    \centering
    \begin{tabular}{r|lllllll}
    \hline
     Setting & $d_i$ & $\Delta_i$ & $\bigstar_i^2$ & $\bigstar_i^4$ & $\dagger_i^k$ & $B_i$ & $C_i$ \\ 
     \hline
        1    & 0 & 10 & 0 & 0 & 0 & 0 & 0\\
        2    & 10 & 10 & 0 & 0 & 0 & 0 & 0\\
        3    & 0 & 1 & 10 & 1 & 1 & 1 & -1\\
        4    & 5 & 1 & 10 & 1 & 1 & 1& -1\\
        \hline
    \end{tabular}
    \caption{Weights used for interference parameters in Experiment 2.}
    \label{Tab:SettingsAdditive}
\end{table}

Results for this experiment are presented in Figure \ref{Fig:Additive}. 
From the figure, we see that FLAME-Networks performs relatively well in most of the settings considered, but other methods do better in some settings. In Settings 1 and 3, representing both simple and complex interference functions, respectively, FLAME-Networks either performs on par with other methods or outperforms them. When degree is introduced to these interference functions (Settings 2 and 4), all competing estimators perform better, relative to FLAME-Networks. In particular, the performance of the SANIA and stratified estimators improves dramatically when degree is introduced into the interference function. This is expected for the stratified estimator as in Setting 4 it is stratifying on the correct feature. The SANIA estimator also seems to capitalize upon the importance of degree, and this is due to it being relatively similar to the stratified degree estimator in our context. 
% From the figure, we see that FLAME-Networks performs well in all the settings considered. In Setting 1, when interference is induced by a feature that is not a subgraph count, FLAME performs well; presumably matching on all subgraph counts allows it to approximate the relevant feature. On the other hand, when the interference is a simple function of a single subgraph (Setting 2), FLAME-Networks is able to identify the feature of interest and also performs very well. Setting 3 introduces a more complex interference function and once more, FLAME performs competitively. When degree is introduced to this interference function (Setting 4), however, all competing estimators to perform better, relative to FLAME-Networks, than they did in Setting 3.
% From the figure we can see that FLAME-Networks performs well in all the settings considered. When the interference function is simple (Settings 1 and 2) simple methods like matching on eigenvalues or degree-stratified estimators also work well (we note that node degree is correlated with the first eigenvector of the adjacency matrix, while the number of triangles one belongs to is a function of all $n$ eigenvectors \citep{tsourakakis2011counting}). However, when interference becomes more complex (Settings 4 and 5) these estimators also start to perform poorly, while FLAME-Networks maintains good performance, relative to the signal to noise ratio in the observed outcome.
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=.8\linewidth]{figures/final_additive.png}
    \caption{Results from experiments with an additive interference function.  Each violin plot represents the distribution of absolute estimation error over simulations for each method. The panels are numbered according to the parameter setting the simulations were ran with. Violin plots are color-coded blue if the method had mean error either equal or better than FLAME-Networks and red otherwise. The black line inside each violin is the median error. The dashed line is FLAME-Networks' mean error.}
    \label{Fig:Additive}
\end{figure}

% The stratified estimator does well in two of the settings above: first, when interference is simple and degree matters (Setting 2), and second when interference is complex without degree (Setting 4). In the first case, the stratified estimator is expected to perform well, as it is stratifying on the correct set of subgraphs for that interference generation. In the second setting, it is likely that degree is correlated with combinations of the other interference components.
